Hypersphere Secure Sketch Revisited: Probabilistic Linear Regression Attack on IronMask in Multiple Usage

Protection of biometric templates is a critical and urgent area of focus. IronMask demonstrates outstanding recognition performance while protecting facial templates against existing known attacks. In high-level, IronMask can be conceptualized as a fuzzy commitment scheme building on the hypersphere directly. We devise an attack on IronMask targeting on the security notion of renewability. Our attack, termed as Probabilistic Linear Regression Attack, utilizes the linearity of underlying used error correcting code. This attack is the first algorithm to successfully recover the original template when getting multiple protected templates in acceptable time and requirement of storage. We implement experiments on IronMask applied to protect ArcFace that well verify the validity of our attacks. Furthermore, we carry out experiments in noisy environments and confirm that our attacks are still applicable. Finally, we put forward two strategies to mitigate this type of attacks.

==> algorithms/null-vector-attack-k.tex <==
\begin{algorithm}[!tbp]
    \caption{Null Vector Attack on $k>(n-1)$ matrices}\label{alg:nva-kk}
    \scriptsize
    \begin{algorithmic}[1]
        \Require Matrices $\mtx M_1, \mtx M_2, \ldots, \mtx M_{k} \in O(n)$, threshold $\theta_t$
        \Ensure $w$ satisfies that $\mtx M_1 w,\mtx M_2 w, \ldots, \mtx M_{k} w \in \mathcal C_\alpha$
        \Repeat 
            \For{$i=1, \dots, k$}
                \State $\vect v_i^T \gets$ Random select row vector of $\mtx M_i$;
            \EndFor
            \State $\mtx M \gets$ vertical stack of $\vect v_1^T, \vect v_2^T, \ldots, \vect v_{k}^T$;
            \State \textcolor{red}{Compute the right singular vector $\vect w'=(w_1, \ldots, w_n)$ with smallest singular value of $\mtx M$;}
            \State $\vect c \gets \mtx M_1 \vect w'$;
            \State $\vect c' \gets \mathbf{Decode}(\vect c)$;
        \Until{$Angle(\vect c, \vect c') < \theta_t$}
        \State $\vect w \gets \mtx M_1^{-1} \vect c'$
        \State \Output $\vect w$
    \end{algorithmic}
\end{algorithm}

==> tables/ecc.tex <==
\begin{table}[!htbp]
    \caption{HyperSphere secure sketch based on the construction in Definition \ref{def:hyper-ecc-becc}. The chosen binary ECC code is BCH code.}\label{tab:ecc}
    \centering
    \begin{tabular}[t]{|c|c|c|c|c|}
        \hline 
        \multicolumn{2}{|c|}{BCH(511, k, t)} & \multirow{2}{*}{$\frac{\theta}{2}$} & \multirow{2}{*}{$\frac{\theta_e}{2}$} & \multirow{2}{*}{\#Security bit} \\
        \cline{1-2}
        $k$ & $t$ & & & \\
        \hline
        322 & 22 & $16.9^{\circ}$ & $29^{\circ}$ & 322 
        \\
        \hline
        304 & 25 & $18.0^{\circ}$ & $30^{\circ}$ & 304 
        \\
        \hline
        259 & 30 & $19.7^{\circ}$ & $31^{\circ}$ & 259 
        \\
        \hline
        241 & 36 & $21.6^{\circ}$ & $32^{\circ}$ & 241 
        \\
        \hline
        211 & 41 & $23.1^{\circ}$ & $34^{\circ}$ & 211 
        \\
        \hline
        175 & 46 & $24.5^{\circ}$ & $37^{\circ}$ & 175 
        \\
        \hline
    \end{tabular}
    \begin{tabular}[t]{|c|c|c|c|c|}
        \hline 
        \multicolumn{2}{|c|}{BCH(511, k, t)} & \multirow{2}{*}{$\frac{\theta}{2}$} & \multirow{2}{*}{$\frac{\theta_e}{2}$} & \multirow{2}{*}{\#Security bit} \\
        \cline{1-2}
        $k$ & $t$ & & & \\
        \hline
        130 & 55 & $26.8^{\circ}$ & $39^{\circ}$ & 130 
        \\
        \hline
        112 & 59 & $27.8^{\circ}$ & $39.6^{\circ}$ & 112 
        \\
        \hline
        94 & 62 & $28.5^{\circ}$ & $40.7^{\circ}$ & 94 
        \\
        \hline
        67 & 87 & $33.9^{\circ}$ & $46.5^{\circ}$ & 67 
        \\
        \hline
        31 & 109 & $38.1^{\circ}$ & $51.6^{\circ}$ & 31 
        \\
        \hline
    \end{tabular}
\end{table}

==> tables/error_prone.tex <==
\begin{table}[!tbp]
    \caption{The number of iterations(Scalar) to terminate across different parameters $\theta'$ and $\theta_t$ with the condition that the assumption $\mathcal A$ in section \ref{ch:nva-details} is true. $\prob{Success}$ indicates the probability that the output template is original template.}\label{tab:scalar-error}
    \centering
    \begin{tabular}{|l|c|c|c|c|c|c|}
        \hline 
        \multirow{2}{*}{$\theta'$} & \multicolumn{3}{c|}{Algorithm \ref{alg:nva-n}} & \multicolumn{3}{c|}{Algorithm \ref{alg:nva-2}}\\
        \cline{2-7}
        & $\theta_t$& Scalar & \prob{Success} & $\theta_t$ & Scalar & \prob{Success} \\
        \hline
        $2.8^{\circ}$ & \multirow{4}{*}{$47^{\circ}$} & $3.0$ & $99\%$ & \multirow{4}{*}{$37^{\circ}$} & $1.2$ & $97\%$ \\
        \cline{1-1}\cline{3-4}\cline{6-7} 
        $5.6^{\circ}$ &  & $8.3$ & $96\%$ & & $6.7$ & $97\%$ \\
        \cline{1-1}\cline{3-4}\cline{6-7} 
        $8.5^{\circ}$ &  & $44$ & $89\%$ &  & $34$ & $93\%$ \\
        \cline{1-1}\cline{3-4}\cline{6-7} 
        $11^{\circ}$ &  & $128$ & $85\%$ &  & $346$ & $84\%$ \\
        \hline
        $14^{\circ}$ & $50^{\circ}$ & $1528$ & $50\%$ & \multirow{2}{*}{$43^{\circ}$} & $277$ & $31\%$ \\
        \cline{1-4}\cline{6-7}
        $19^{\circ}$ & - & - & - & & $9953$ & $18\%$ \\
        \hline
    \end{tabular}
\end{table}

==> tables/error_prone_kversion.tex <==
\begin{table}[tbp]
    \caption{Estimated expected runtime for different parameters $\theta', \theta_t, k$. $\#iters$ is the expected number of iterations to obtain correct matrix $\mtx M$ without noise. The Scalar and $\prob{Success}$ are same as in Table \ref{tab:scalar-error}. The estimated expected runtime(Time) is calculated by $Scalar * \#iters * \text{time per iter} / \prob{Success}$.}\label{tab:scalar-error-k}
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
        \hline 
        $\theta'$ & $\theta_t$ & k & Scalar & $\prob{Success}$ & \#iters & time per iter &  Time\\
        \hline
        $8.5^{\circ}$ & $49^{\circ}$ & 561  & 1 &  $100\%$ & $5\times 10^7$ & 41 ms & 25 day \\
        \hline
        $11^{\circ}$ & $49^{\circ}$ & 561  & 1 &  $100\%$ & $5\times 10^7$ & 41 ms & 25 day \\
        \hline
        $14^{\circ}$ & $49^{\circ}$ & 561 & 1.37 &  $93\%$ & $8\times 10^7$ & 41 ms & 37 day \\
        \hline
        $19^{\circ}$ & $49^{\circ}$ & 611 & 1.45 &  $88\%$ & $4\times 10^8$ & 43 ms & 218 day \\
        \hline
        $26^{\circ}$ & $49^{\circ}$ & 731 & 1.26 &  $88\%$ & $1.7\times 10^{10}$ & 50 ms & 27 year \\
        \hline
        $30^{\circ}$ & $53^{\circ}$ & 731 & 2.73 &  $37\%$ & $8\times 10^{10}$ & 50 ms & 140 year \\
        \hline
        $36^{\circ}$ & $50^{\circ}$ & 961 & 2.02 &  $55\%$ & $6.5\times 10^{13}$ & 58 ms & $1.0\times 10^{5} $ year \\
        \hline
    \end{tabular}
\end{table}

==> tables/expected_time.tex <==
\begin{table}[htbp]
    \caption{The number of iterations and estimated runtime for successfully recovering template $\vect w$ or $-\vect w$ with an expected value of 1 are analysed across different parameters $\alpha$ with fixed $n=512$ for Algorithm \ref{alg:nva-n} and Algorithm \ref{alg:nva-2}. The estimated runtime is determined by the product of the execution time of \algo{null\_space} and the number of iterations. The experimental $\frac{\theta_e}{2}$ indicates the practical error correcting capacity in Definition \ref{def:hyper-ecc}. It demonstrates that the probability of $\algo{Decode}(\vect a) = \vect c$ is larger than $50\%$ if $Angle(\vect a, \vect c) < \frac{\theta_e}{2}$, average on 100 tests with randomness of $\vect a, \vect c$ and sketch $\mtx M$.} \label{tab:expected-time}
    \centering
    \begin{tabular}{|r|c|c|c|c|c|c|c|}
        \hline 
        \multirow{2}{*}{$\alpha$} & \multicolumn{2}{c|}{Algorithm \ref{alg:nva-n}} & \multicolumn{2}{c|}{Algorithm \ref{alg:nva-2}} & \multirow{2}{*}{$\frac{\theta}{2}$} & \multirow{2}{*}{$\frac{\theta_e}{2}$} & \multirow{2}{*}{\#Security bit} \\
        \cline{2-5}
        & \#iters & Time & \#iters & Time & &  & 
        \\
        \hline
        4 & 54 & 2.2 s & 258 & 2.2 s & $20^{\circ}$ & $66^{\circ}$ & $35$ \\
        8 & $3\times10^4$ & 2.1 min & $7\times10^4$ & 10 min & $14^{\circ}$ & $59.7^{\circ}$ & $64$ \\
        12 & $2\times10^5$ & 2.1 hour & $2\times10^8$ & 2 day & $11^{\circ}$ & $53.4^{\circ}$ & $90$ \\
        16 & $1\times10^7$ & 5.3 day & $6\times10^{9}$ & 1.7 year & $10^{\circ}$ & $48^{\circ}$ & $115$ \\
        20 & $7\times10^8$ & 1 year & $2\times10^{12}$ &  582 year & $9.1^{\circ}$ & $42^{\circ}$ & $138$ \\
        24 & $4\times10^{10}$ & 58 year & $7\times10^{14}$ & > $10^6$ year & $8.3^{\circ}$ & $37^{\circ}$ & $160$ \\
        36 & $2\times10^{16}$ & > $10^8$ year & $5\times10^{22}$ & > $10^{14}$ year & $6.7^{\circ}$ & $31^{\circ}$ & $220$ \\
        \hline
    \end{tabular}
\end{table}

==> tables/null_space_running_time.tex <==
\begin{table}[htbp]
    \caption{The average Running time of \algo{null\_space} on 1000 times with diffreent matrix shapes.}\label{tab:null_space_running_time}
    \centering
    \begin{tabular}{|l|c|c|}
        \hline 
        Matrix Shape & 255 * 256 & 511 * 512 \\
        \hline
        Running time & 8.4ms & 41ms \\
        \hline
    \end{tabular}
\end{table}
